Mean Estimation with Sub-Gaussian Rates in Polynomial Time

We study polynomial time algorithms for estimating the mean of a heavy-tailed multivariate random vector. We assume only that the random vector $X$ has finite mean and covariance. In this setting, the radius of confidence intervals achieved by the empirical mean are large compared to the case that $X$ is Gaussian or sub-Gaussian. We offer the first polynomial time algorithm to estimate the mean with sub-Gaussian-size confidence intervals under such mild assumptions. Our algorithm is based on a new semidefinite programming relaxation of a high-dimensional median. Previous estimators which assumed only existence of finitely-many moments of $X$ either sacrifice sub-Gaussian performance or are only known to be computable via brute-force search procedures requiring time exponential in the dimension.

==> content/2-to-1-norm.tex <==
\section{Certifying the Median}
In this section we prove \cref{lem:sos-med-2}, showing that constant degree SoS proofs certify upper bounds on a certain high-dimensional median.
The starting point is the following simple fact, allowing us to exchange optimization over $\pE \|\mu - y\|^2$ for optimization over $\pE \sum b_i$.

\begin{fact}
  Let $\cU$ be a set and let $f,g \, : \, \cU \rightarrow \R$.
  Suppose that
  $
  \max_{\substack{x \in \cU \\ g(x) \geq a}} f(x) \leq b\
  $.
  Then
  $
  \max_{\substack{x \in \cU \\ f(x) \geq b}} g(x) \leq a\mper
  $
\end{fact}
\begin{proof} The second statement is the contrapositive of the first. \end{proof}

Our first lemma offers a reformulation of the bound we aim to prove as a natural median certification problem over the unit sphere.

\begin{lemma}\label[lemma]{lem:rescale}
  Let $Z_1,\ldots,Z_k \in \R^d$.
  Let $\cP(r,Z_1,\ldots,Z_k)$ be the following system of inequalities:
  \begin{align*}
    b_i^2 = b_i, \quad b_i(\iprod{Z_i,x} - \|x\|^2) \geq 0, \quad \|x\|^2 = r^2\mper
  \end{align*}
  Let $\cQ(r,Z_1,\ldots,Z_k)$ be the following system of inequalities:
  \[
  b_i^2 = b_i, \quad b_i \iprod{Z_i,x} \geq b_i r, \quad \|x\|^2 = 1
  \]
  Then over degree $4$ pseudodistributions, $\max_{\pE \text{ satisfies } \cP} \sum_{i \leq k} b_i \leq \max_{\pE \text{ satisfies } \cQ} \sum_{i \leq k} b_i$.
\end{lemma}
\begin{proof}
  Let $\pE$ satisfy $\cP$.
  Consider the change of variables $y = \tfrac 1r x$.
  The psuedodistribution given by $\pE p(b,y) = \pE p(b,\tfrac 1r x)$ satisfies $\pE \|y\|^2 = 1$, and note that if $\|x\|^2 = r$ then $b_i(\iprod{Z_i,x} - \|x\|^2) \geq 0$ rearranges to $b_i \iprod{Z_i,y} \geq b_i r$.
  So we have obtained a pseudodistribution satisfying $\cQ$ with $\pE \sum_{i \leq k} b_i$ unchanged.
\end{proof}


The next two lemmas are the heart of the proof; we prove them in the following subsections.
The following analyes the expected maximum of $\pE \sum b_i$, where the expectation is over $Z_1,\ldots,Z_k$.

\begin{lemma}[Expectation]
\label[lemma]{lem:expectation}
  Let $Z_1,\ldots,Z_k \in \R^d$ be i.i.d. copies of a random variable $Z$ with $\E Z = 0$ and $\E ZZ^\top = \Sigma$.
  Let $r \geq 24 \sqrt{\Tr \Sigma / k} + 24 \sqrt{\|\Sigma\|}$.
  Let $\cQ(r,Z_1,\ldots,Z_k)$ be as in \cref{lem:rescale}.
  Then
  \[
  \E_{Z_1,\ldots,Z_k} \Brac{\max_{\substack{\pE \text{ degree 4},\\\text{satisfies } \cQ}} \pE \sum_{i \leq k} b_i } \leq \frac k8\mper
  \]
\end{lemma}

The last lemma will allow us to prove exponential concentration about the mean for $\max_{\substack{\pE \text{ degree 4},\\\text{satisfies } \cQ}} \pE \sum_{i \leq k} b_i$.

\begin{lemma}[Bounded Differences]
\label[lemma]{lem:concentration}
  Let $z_1,\ldots,z_k \in \R^d$ and $r > 0$.
  Let $i \in [k]$ and let $z_i' \in \R^d$.
  Then
  \[
  \Abs{\max_{\substack{\pE \text{ degree } 4\\\text{and satisfies } \cQ(r,z_1,\ldots,z_k)}} \pE \sum_{i \leq k} b_i
  - \max_{\substack{\pE \text{ degree } 4\\\text{and satisfies } \cQ(r,z_1,\ldots,z_i',\ldots,z_k)}} \pE \sum_{i \leq k} b_i } \leq 1\mper
  \]
\end{lemma}
\begin{proof}[Proof of \cref{lem:concentration}]
  For brevity, let $\cQ = \cQ(r,z_1,\ldots,z_k)$ and $\cQ' = \cQ(r,z_1,\ldots,z_i',\ldots,z_k)$.
  It will suffice to show that if $\pE$ satisfies $\cQ$, then there is $\pE'$ which satisfies $\cQ'$ such that $\pE \sum_{i \leq k} b_i \leq \pE' \sum_{i \leq k} b_i + 1$.
  Let $\pE$ satisfy $\cQ$.
  Then let $\pE''$ be the restriction of $\pE$ to the variables $b_1,\ldots,b_{i-1},b_{i+1},\ldots,b_k,x$, and $\pE'$ be the product of $\pE$ with the distribution on $b_i$ which sets $b_i =0$ with probability $1$.
  Then for all $j \neq i$ we have $\pE b_j =\pE' b_j$, and since $\pE b_i \leq 1$ we are done.
\end{proof}

Now we can prove \cref{lem:sos-med-2}.

\begin{proof}[Proof of \cref{lem:sos-med-2}]
\Snote{TODO: fix, and fix the constants}
  By \cref{lem:expectation}, if $r \geq 24(\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$ then we have $\E m(Z_1,\ldots,Z_k,r) \leq k/8$.
  On the other hand, by the bounded differences inequality and \cref{lem:concentration}, we have $\Pr(m - \E m > t) \leq \exp(-2t^2/k)$.
  Setting $t = k/8$ we find that $\Pr(m > k/4) \leq \exp(k/32)$.
  Now the lemma follows by duality of SoS proofs and pseudodistributions.
\end{proof}


\subsection{Expectation Step}
In this section we prove \cref{lem:expectation}.
\subsection{Concentration Step}

In this section we prove \cref{lem:concentration}.

\begin{proof}[Proof of \cref{lem:concentration}]
  For brevity, let $\cQ = \cQ(r,z_1,\ldots,z_k)$ and $\cQ' = \cQ(r,z_1,\ldots,z_i',\ldots,z_k)$.
  It will suffice to show that if $\pE$ satisfies $\cQ$, then there is $\pE'$ which satisfies $\cQ'$ such that $\pE \sum_{i \leq k} b_i \leq \pE' \sum_{i \leq k} b_i + 1$.
  Let $\pE$ satisfy $\cQ$.
  Then let $\pE''$ be the restriction of $\pE$ to the variables $b_1,\ldots,b_{i-1},b_{i+1},\ldots,b_k,x$, and $\pE'$ be the product of $\pE$ with the distribution on $b_i$ which sets $b_i =0$ with probability $1$.
  Then for all $j \neq i$ we have $\pE b_j =\pE' b_j$, and since $\pE b_i \leq 1$ we are done.
\end{proof}






==> content/bdd-differences.tex <==
\section{Bounded Differences for SoS Median}




==> content/explicit-sdp.tex <==
\section{An explicit SDP} \label[section]{sec:explicit-sdp}
In this section we record an explicit semidefinite program whose solutions are the feasible pseudodistributions for \textsc{median-sdp}.
This construction is not novel: the ideas originate with Lasserre, Parillo, Nesterov, and Shor \cite{lasserre2001global, shor1987approach, parrilo2000structured, nesterov2000squared}, and the correspondence between SDPs and pseudodistributions has become standard in the Sum of Squares optimization and algorithms literature.


We define two sets of PSD matrices, corresponding to the pseudodistributions $\pE$ and $\pE'$ in \textsc{median-sdp}.
We start with $\pE'$, which will correspond to an SDP we call \textsc{inner-sdp}.

\paragraph{\textsc{inner-sdp}}
The variables in our semidefinite program are indexed by triples of multi-indices $(\alpha,\beta,\gamma)$ where $\alpha,\beta$ are over $[d]$ and $\gamma$ is over $[k]$, and $|\alpha| + |\beta| + |\gamma| \leq 4$.
For each, we introduce a variable $Y_{\alpha,\beta,\gamma}$.
To obtain the operator $\pE'$ of \textsc{median-sdp} from the variables $Y$, set $\pE' x^\alpha v^\beta b^\gamma = Y_{\alpha,\beta,\gamma}$, and linearly to all degree $4$ polynomials in $x,b,v$.
Throughout suppose $Z_1,\ldots,Z_k \in \R^d$.

The SDP involves several families of constraints on these variables.
The first will enforce that $\pE'$ satisfies $b_i^2 -b_i =0$.
\begin{align*}
\tag{Boolean constraints} Y_{\alpha,\beta,\gamma} = Y_{\alpha,\beta,\gamma'} \text{ if $\gamma = \gamma'$ as \emph{subsets of } [k]}\mper
\end{align*}
(Note the important distinction between sets and multisets.)
The next will enforce that $\pE'$ satisfies $\sum b_i = k/2$.
\begin{align*}
& \tag{Size constraints} \sum_{i \leq k} Y_{\alpha,\beta,\gamma \cup \{i\}} = \frac k2 \sum_{i \leq k} Y_{\alpha,\beta,\gamma} \text{ if $|\alpha| + |\beta| + |\gamma| \leq 3$}\mper
\end{align*}
The third set enforces that $\pE' b_i \iprod{Z_i - x,v} \geq \pE' b_i \|v\|^2$.
\begin{align*}
& \tag{Threshold constraints} \sum_{j \in [d]} Z_{ij} Y_{\emptyset,\{j\},\{i\}} - \sum_{j \in [d]} Y_{\{j\},\{j\},\{i\}} \geq \sum_{j \in [d]} Y_{\emptyset,\{j,j\},\{i\}} \text{ for all $i \leq k$} \mper
\end{align*}
The final linear constraint enforces normalization:
\begin{align*}
& \tag{Normalization constraint} Y_{\emptyset,\emptyset,\emptyset} = 1\mper
\end{align*}
Finally, let $M$ be the matrix with rows and columns indexed by $(\alpha,\beta,\gamma)$ such that $|\alpha| + |\beta| + |\gamma| \leq 2$, with
\begin{align*}
M_{(\alpha,\beta,\gamma),(\alpha',\beta',\gamma')} = Y_{\alpha \cup \alpha', \beta \cup \beta', \gamma \cup \gamma'}\mper
\end{align*}
Then
\begin{align*}
& \tag{Positivity constraint}  M \succeq 0\mper
\end{align*}
One approach treats $Y$ as the SDP variables and $M$ as a matrix of linear forms in those variables; this is enough to solve the SDP with most methods.
If writing the SDP in the canonical form \cref{eq:sdp}, then the matrix $M$ is the SDP variable, and all the constraints on $Y$ translate to appropriate linear constraints on $M$.
In addition, to ensure that each $M$ uniquely defines values for $Y$, so-called \emph{SoS symmetry} constraints must be added:
\begin{align*}
& M_{(\alpha_0,\beta_0,\gamma_0),(\alpha_0',\beta_0',\gamma_0')} = M_{(\alpha_1,\beta_1,\gamma_1),(\alpha_1',\beta_1',\gamma_1')} \text{ if }\\
& \alpha_0 \cup \beta_0 \cup \gamma_0 \cup \alpha_0' \cup \beta_0' \cup \gamma_0' = \alpha_1 \cup \beta_1 \cup \gamma_1 \cup \alpha_1' \cup \beta_1' \cup \gamma_1' \text{ as multisets.}
\end{align*}

\paragraph{\textsc{outer-sdp}}
We move on to the SDP corresponding to $\pE$ in \textsc{median-sdp}.
Let \textsc{outer-sdp} be the set $(X_\alpha)_{|\alpha| \leq 4}$ where $\alpha$ is a multi-index over $[d]$ such that
\[
  X_{\emptyset, \emptyset} = 1 \text{ and } (X_{\alpha \cup \alpha'})_{\alpha,\alpha'} \succeq 0\mper
\]



\paragraph{Solution via ellipsoid algorithm}

Recalling the definitions of \textsc{inner-sdp} and \textsc{outer-sdp} from the last section, \textsc{median-sdp} can be written as
\[
  \min_{X \in \textsc{outer-sdp}} \max_{\substack{Y \in \textsc{inner-sdp} \\ Y_{\alpha,\emptyset,\emptyset} = X_{\alpha}}} \sum_{i \leq d} Y_{\emptyset, \{i,i\}, \emptyset}\mper
\]
It is not hard to check that the function
\[
f(X) = \max_{\substack{Y \in \textsc{inner-sdp} \\ Y_{\alpha,\emptyset,\emptyset} = X_{\alpha}}} \sum_{i \leq d} Y_{\emptyset, \{i,i\}, \emptyset}
\]
is convex.
Furthermore, it can be computed to accuracy $\e$ in time $(dk \log (1/\e))^{O(1)}$ by standard semidefinite programming solving algorithms.
Thus by the ellipsoid method (see e.g Theorem 4.3.13 of \cite{grotschel2012geometric}) applied to $\min_{X \in \textsc{outer-sdp}} f(X)$ it is possible to solve \textsc{median-sdp} in polynomial time.


==> content/graveyard.tex <==

To construct our final estimation algorithm, we use the following meta-theorem on estimation via SoS proofs.
Informally, the theorem says that a degree-$t$ SoS identifiability proof of parameters $\theta$ from samples $X_1,\ldots,X_n$ from a probability distribution $P_\theta$ can be turned into an algorithm to estimate $\theta$ with running time $n^{O(t)}$.
This meta-theorem and others similar to it are at the heart of most recent SoS-based algorithms for parameter estimation.
For completeness we provide a proof in the appendix, though it involves no new ideas.

\begin{theorem}[SoS meta-theorem on parameter estimation]
\label[theorem]{thm:sos-meta}
  There is a universal constant $C$ such that the following is true.
  Let $P_{\theta,\theta'}(x)$ be a family of probability distributions on $\R^n$, parameterized by $\theta \in \R^m$ (the parameters to be estimated) and $\theta'$ (auxiliary parameters).
  Suppose for some $N,t \in \N$ and $\epsilon,\delta > 0$ there is a family of $N$ polynomial inequalities $p_1(y,w,x) \geq 0,\ldots,p_N(y,w,x) \geq 0$ in variables $y=y_1,\ldots,y_m$, $w=w_1,\ldots,w_M$ and $x = x_1,\ldots,x_n$ such that for every $\theta \in \R^d$ and every $\theta'$, with probability $1-\delta$ over i.i.d. $X \sim P_{\theta,\theta'}$, there is a degree $t$ SoS refutation of
  \[
    \left \{ p_1(y,w,X) \geq 0,\ldots,p_N(y,w,X) \geq 0, \|y - \theta\|^2 \geq \e^2  \right \}
  \]
  with coefficients bounded by $B > 0$.\footnote{It is for convenience that $p_i$ is a polynomial in $X$; it would suffice that there is an efficient algorithm which takes $X$ as input and outputs a list of coefficients of the polynomial $p_i(y,w,X)$ in variables $y,w$.}
  Then for every $\e' > 0$ there is an algorithm with running time $((n+m+M) \cdot N \cdot \log \tfrac {1}{\e'})^{Ct}$ which with probability $1-\delta$ over input $X_1,\ldots,X_n \sim P_{\theta,\theta'}(x)$ produces a vector $\hat{\theta} \in \R^d$ with $\|\hat{\theta} - \theta\| \leq \e + B \e'$.
\end{theorem}

Our main theorem follows from \cref{thm:sos-meta} and the following lemma, which asserts the existence of an SoS identifiability proof for mean estimation.

\begin{lemma}\label[lemma]{lem:main}
  Let $d \in \N$ and let $\cP$ be the class of probability distributions on $\R^d$ with finite first and second moments.
  For every $n \in \N$ and $\delta > 0$ there is a family of $N \leq (nd)^{O(1)}$ polynomials $\{p_i(y,w,x_1,\ldots,x_n)\}_{i \in [N]}$ in variables $y = y_1,\ldots,y_d$, $w_1,\ldots,w_m$ for $m \leq (nd)^{O(1)}$ such that for every $P \in \cP$, with probability at least $1-\delta$ over i.i.d. $X_1,\ldots,X_n \sim P$, there is a degree-$O(1)$ SoS refutation of
  \[
    \left \{ p_i(y,w,X_1,\ldots,X_n) \geq 0 \right \}_{i \in [N]} \cup \left \{ \|y-\mu\|^2 \geq 128 \Paren{\sqrt{\frac{\Tr \Sigma}{n}} + \sqrt{\frac{\|\Sigma\| \log \tfrac 1 \delta}{n}} } \right \}
  \]
  with coefficients bounded by $(n \cdot d \cdot \max_{i \leq n} \|X_i\|)^{O(1)}$, where $\mu = \E_{X \sim P} X$ and $\Sigma = \E_{X \sim P}(X - \mu)(X - \mu)^\top$.
\end{lemma}



\section{SoS Identifiability via the Median}

In this section we prove \cref{lem:main}.
The main idea is that the polynomials $p_i(y,w,X_1,\ldots,X_n)$

In this section we describe our main algorithm and analyze it.
The starting point is the following polynomial system.

\begin{definition}\label[definition]{def:median-polys}
  Let $\bZ = Z_1,\ldots,Z_k \in \R^d$ and $r > 0$.
  Solutions to the polynomial system $\cM_{\bZ,r}$ are vectors $\mu \in \R^d$ such that for any $x \in \R^d$, if $\|x - Z_i\| \leq \|\mu - Z_i\|$ for more than $k/2$ indices $i \in [k]$ then $\|x - \mu\| \leq r$.
  (The system also involves some auxiliary variables.)
\end{definition}



\section{OLD INTRODUCTION}
So we ask: is it possible to estimate the mean of $X$ via some estimator with guarantees similar to \eqref{eq:gauss-concentration} when $X$ is heavy-tailed?


We address a simple problem: given i.i.d. copies $X_1,\ldots,X_n$ of an unknown random vector $X \in \R^d$ with finite mean $\mu$ and covariance $\Sigma$, and an error tolerance $\delta > 0$, find an estimate $\hat{\mu}_\delta(X_1,\ldots,X_n)$ such that $\Pr \{ \|\hat{\mu} - \mu\| > r_\delta \} \leq \delta$ for as small a number $r_\delta$ as possible.
Our main result is the first polynomial-time algorithm for this problem which achieves essentially optimal confidence radius $r_\delta$ (up to constant factors).

Our goal is to design an estimator which is both statistically and computationally efficient.
For us, that means it should achieve essentially optimal rates of statistical error and also be computable in polynomial time.

We emphasize that the running time of our algorithm is polynomial in both $n$, the number of samples, and $d$
Our algorithm is based on semidefinite programming.

Under only the assumption that $X$ has finite covariance, the samples $X_1,\ldots,X_n$ may contain many outliers.
Consider their effect on the empirical mean $\overline{\mu}_n = \tfrac 1n \sum_{i \leq n} X_i$.
While among all estimators $\overline{\mu}_n$ minimizes the mean squared error, $\E \|\mu - \overline{\mu}_n \|^2 = \Tr \Sigma / n$, the concentration of $\|\mu - \overline{\mu}_n\|$ may be rather poor.
Chebyshev's inequality shows that 
\[
\Pr\left \{ \Norm{\mu - \overline{\mu}_n} > \sqrt{\frac{ \Tr \Sigma }{\delta n}} \right \} \leq \delta\mper
\]
By constructing $X$ where outliers at radius $\Tr{\Sigma / \sqrt{\delta}}$ occur with probability of order $\delta$ one may see that this analysis of the empirical mean is tight.

If $X$ were Gaussian, however, the story would be different.
By applying Gaussian concentration to $\|\mu - \overline{\mu}_n\|$, one may show that
\begin{align}
  \Pr \left \{ \Norm{\mu - \overline{\mu}_n} > \sqrt{\frac{\Tr \Sigma}{n}} + \sqrt{\frac{2 \|\Sigma\| \log(1/\delta)}{n}} \right \} \leq \delta\mcom \label[equation]{eq:subgauss}
\end{align}
where $\|\Sigma\| = \lambda_{\max}(\Sigma)$ is the maximum eigenvalue of $\Sigma$.
This bound is improved in two ways: the $1/\delta$ term has become $\log(1/\delta)$, and that term multiplies $\|\Sigma\|$ rather than $\Tr \Sigma$, which may may differ by a factor of the dimension $d$.
Following \cite{LM18}, we say that an estimator which achieves \cref{eq:subgauss} (up to a constant factor) has \emph{sub-Gaussian performance}.



\paragraph{Previous polynomial time estimators}
As we have already discussed, while it is trivially computable in polynomial time, the empirical mean is far from achieving sub-Gaussian performance under the assumptions of \cref{thm:main}
Naive outlier removal -- discarding samples $X_i$ with large norms $\|X_i\|$ before computing the empirical mean -- is more successful.
However, it is not a translation-invariant operation, so while the first-order growth rate of the confidence radius it achieves is sub-Gaussian, the radius depends at second order on $\E \|X\|^2$ rather than $\E \|X - \mu\|^2 = \Tr \Sigma$ \cite{catoni2018dimension}.

The previous polynomial-time estimator which comes closest to sub-Gaussian performance under the same assumptions as \cref{thm:main} is Minkser's geometric median algorithm \cite{minsker2015geometric}.
The geometric median of $Z_1,\ldots,Z_k \in \R^d$ is
\[
\text{geometric-median}(Z_1,\ldots,Z_k) = \arg \min_{x \in \R^d} \sum_{i \leq k} \|Z_i - x\|\mper
\]
Minsker proves that if $Z_1,\ldots,Z_k$ are each the average of $n/k$ samples $X_i$ for $k = \Theta(\log 1/\delta)$ then
\[
  \Pr \left \{ \Norm{\text{geometric-median}(Z_1,\ldots,Z_k) - \mu} > C \sqrt{\frac{\Tr \Sigma \cdot \log(1/\delta)}{n}} \right \} \leq \delta
\]
for some universal constant $C$.

A result of Cohen et al. shows that $\text{geometric-median}(Z_1,\ldots,Z_k)$ is computable in nearly-linear time (that is, time $dk \cdot (\log dk)^{O(1)}$ -- slower but still polynomial time algorithms were known previously) \cite{DBLP:conf/stoc/CohenLMPS16}.
\cref{thm:main} of this work improves on the geometric median by moving the $\log(1/\delta)$ term to multiply $\|\Sigma\|$ rather than $\Tr \Sigma$, matching the performance of the empirical mean in the Gaussian setting.
Recall that $\Tr \Sigma$ may be as large as $d \|\Sigma\|$ if $X$ is isotropic.
In modern settings, with thousands or millions of dimensions, this difference in the confidence radius is appreciable.


\paragraph{Sub-Gaussian performance, but in exponential time}
Our work has been preceded by substantial exploration of generalizations of the median of means to larger dimensions $d$ \cite{lerasle2011robust,hsu2016loss,minsker2015geometric,LM18}.
The culmination of these works is the median-of-means estimator of Lugosi and Mendelson \cite{LM18}, which was the first to achieve sub-Gaussian performance for arbitrary $d$.
Key to their estimator is a new notion of the $d$-dimensional median of vectors $Z_1,\ldots,Z_k \in \R^d$.
For Lugosi and Mendelson, the median is
\begin{align}
\arg \min_{x \in \R^d} \max_{y \in \R^d} \|x - y \| \text{ such that $\|Z_i - x\| \geq \|Z_i - y\|$ for at least $\tfrac k 2$ $Z_i$'s.}\label[equation]{eq:lm-estimator}
\end{align}
While this estimator achieves sub-Gaussian performance, it is difficult to imagine any computationally-efficient method of evaluating it.
In particular, it appears to require either optimization of a non-convex function in $\R^d$ or combinatorial search through all subsets of the vectors $Z_i$ of size $k/2$.

In numerous well-studied cases, inference problems with similarly combinatorial solutions seem to entirely lack computationally-efficient algorithms.
One major example is the \emph{planted clique} problem, where the goal is to test for the presence of a hidden clique of size about $n^{0.01}$ in an \Erdos-\Renyi graph $G(n,1/2)$.
There is strong evidence from theoretical computer science that no polynomial-time hypothesis testing algorithm substantially beats random guessing for this problem, in spite of the fact that hidden cliques of size $2.01 \log n$ remain detectable if algorithmic considerations are ignored \cite{MR0445898-Karp76, bollobas1976cliques, DBLP:journals/rsa/Jerrum92, DBLP:journals/dam/Kucera95, DBLP:conf/focs/BarakHKKMP16}.
A similar story applies to many more traditional statistics problems: estimation of a sparse principal component of high-dimensional data, for instance \cite{DBLP:conf/isit/AminiW08, krauthgamer2015semidefinite, hopkins2017power}.
Thus prior to this work it was uncertain whether or not there should exist a polynomial time algorithm whose statistical performance matches Lugosi and Mendelson's median of means estimator.

While the algorithm we present does run in polynomial time, it is far from practical on data sets of even moderate dimension, or for moderately small $\delta$.
This is due to the use of a semidefinite programming relaxation which our algorithm solves.
Impractical running times are typical for semidefinite programming based algorithms, until they are further refined.
However, many semidefinite programs in both combinatorial and statistical applications (for example, the classic \textsc{max-cut} semidefinite program \cite{DBLP:journals/jacm/GoemansW95}) are by now known to be solvable in nearly-linear time -- that is, in time $N (\log N)^{O(1)}$ for a size-$N$ input \cite{DBLP:journals/jacm/AroraK16, DBLP:conf/soda/Steurer10, DBLP:conf/stoc/HopkinsSSS16}.
Thus, it seems likely that an algorithm similar to the one we present here can be made truly practical.


\paragraph{Our approach}
Rather than compute \cref{eq:lm-estimator} directly, our approach begins with a convex relaxation.
In particular, we employ a semidefinite program (SDP) from the \emph{Sum of Squares hierarchy}, a powerful family of SDP relaxations for polynomial optimization problems.
Sum of Squares (SoS) SDPs have recently seen numerous applications to computationally-challenging problems in statistics and machine learning.
For instance, they offer the best available polynomial-time guarantees for parameter estimation of high-dimensional mixture models and for estimation in Huber's contamination model \cite{huber1964robust, hopkins2018mixture, kothari2018robust, klivans2018efficient}.
SoS has also been key to progress in computationally-challenging tensor problems with statistical applications, such as tensor decomposition and tensor completion \cite{DBLP:conf/focs/MaSS16, DBLP:conf/colt/BarakM16, potechin2017exact}.

At a high level, our strategy is to show that by choosing a sufficiently strong convex relaxation of \cref{eq:lm-estimator}, the main properties of \cref{eq:lm-estimator} established by Lugosi and Mendelson in the course of proving its sub-Gaussian performance apply also to optimal solutions of the convex relaxation.
Of course, one must be sure that the relaxation does not become so complex that polynomial-time solvability is lost.
The main work in this paper shows that a $(d \cdot \log(1/\delta))^{O(1)}$-size SDP suffices; this is the reason our algorithm runs in polynomial time.



\section{stuff ripped out after round one journal reviews}

We start defining the kind of certificate which certifies that $\mu$ has distance at most $r$ to a median in every direction, with high probability.

\begin{definition}\label[definition]{def:certifiable-percentile}
  Let $Z_1,\ldots,Z_k \in \R^d$.
  For $r > 0$ and $p \in [0,1]$, a point $x \in \R^d$ is a $p$-th $r$-percentile if for every unit vector $v$, there are at most $pk$ vectors $Z_i$ such that $\iprod{Z_i-x,v} > r$.
  If $p = 1/2$ then $x$ is $r$-close to a median in every direction, but we will sometimes take $p < 1/2$.

  The point $x$ is a \emph{certifiable} $p$-th $r$-percentile if there are $\alpha_1,\ldots,\alpha_k, \beta_1,\ldots,\beta_k, \gamma \geq 0$ and a degree $2$ SoS polynomial $\sigma(b,v)$ such that
  \begin{align}\label[equation]{eq:median-certificate}
  pk - \sum_{i=1}^k  b_i & = \sum_{i=1}^k \alpha_i b_i (\iprod{Z_i - x,v} - r)
    + \sum_{i=1}^k \beta_i (1-b_i^2) \\
    & + \gamma (1-\|v\|^2) \nonumber
    + \sigma (b,v)\mper
  \end{align}
  holds as a polynomial identity in variables $b_1,\ldots,b_k,v_1,\ldots,v_d$.
  Finally, $x$ is a \emph{$(c,C)$-nicely certifiable} $p$-th $r$-percentile if furthermore $\gamma \in \{0,1/100,2/100,\ldots,k\}$ and for all $i$ either $\alpha_i = 0$ or $\alpha_i \in [c, C]$.
\end{definition}


Our first main lemma says that if $Z_1,\ldots,Z_k$ are i.i.d. draws from a distribution with bounded covariance then the mean is a nicely certifiable percentile.

\begin{lemma}\label[lemma]{lem:proof-for-mu}
  Let $Z_1,\ldots,Z_k \in \R^d$ be i.i.d. copies of a random vector $Z$ with mean $\mu$ and covariance $\Sigma$.
  Let $r = 1000 (\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$.
  With probability at least $1 - \exp(\Omega(k))$, the mean $\mu$ is a $(\Omega(1/\sqrt{\Tr \Sigma}), O(k/r))$-nicely certifiable $1/10$-th $r$-percentile of $Z_1,\ldots,Z_k$.
\end{lemma}

The second main lemma describes an SoS-based algorithm which takes $Z_1,\ldots,Z_k$ and finds a point close to any nicely certifiable $p$-th percentile (for small enough $p$).


\section{Certifying percentiles for the mean}
\label[section]{sec:sdp-cert}

In this section we prove \cref{lem:proof-for-mu}.
The main problem is to establish that $\mu$ is a certifiable $1/25$-th $r$-percentile.
A small amount of technical work is required to show that if only a small number of vectors $Z_i - \mu$ have norm much larger than $\sqrt{\Tr \Sigma}$ (as occurs with high probability) then $\mu$ is also nicely certifiable, with $1/25$ replaced by $1/10$.
(The choice of constants $1/25 < 1/10 < 1/2$ is arbitrary.)

The first lemma we prove follows directly from duality of pseudodistributions and SoS proofs: it gives a sufficient condition for $\mu$ to be a certifiable $p$-th percentile.

\begin{lemma}\label[lemma]{lem:apply-duality}
  Let $Z_1,\ldots,Z_k \in \R^d$, $r > 0$, and $p \in [0,1]$.
  Let $\mu \in \R^d$.
  Suppose that there is no degree $2$ pseudoexpectation $\pE$ on variables $b_1,\ldots,b_k, v_1,\ldots,v_d$ which has $\pE \sum_{i=1}^k b_i \geq pk$ and satisfies $\{ b_i^2 \leq 1, \|v\|^2 \leq 1, b_i (\iprod{Z_i - \mu,v} - r) \geq 0 \}$.
  Then for every $\e > 0$, $\mu$ is a certifiable $(p+\e)$-th $r$-percentile of $Z_1,\ldots,Z_k$.
\end{lemma}

The next lemma captures the main technical innovations in this section: it shows that the hypothesis of \cref{lem:apply-duality} applies to the mean $\mu$ of $Z_1,\ldots,Z_k$ with high probability.

\begin{lemma}\label[lemma]{lem:mu-is-certifiable}
  Let $Z_1,\ldots,Z_k$ be i.i.d. copies of a random variable $Z$ with mean $\E Z = \mu$ and covariance $\Sigma$.
  Let $r = 1000(\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$.
  With probability at least $1-\exp(-k/2000)$,
  \[
  \max \, \pE \sum_{i =1}^k b_i \leq \frac k {25}
  \]
  where the maximum is taken over degree $2$ pseudodistributions $\pE$ in variables $b_1,\ldots,b_k, v_1,\ldots,v_d$ which satisfy $\cA = \{ \|v\|^2 \leq 1, b_i^2 \leq 1, b_i (\iprod{Z_i-\mu,v} -r) \geq 0 \}$.
\end{lemma}

\subsection{SDP certificates for the mean: \cref{lem:mu-is-certifiable}}
In this section we prove \cref{lem:mu-is-certifiable}.
The proof has two steps, an expectation step and a concentration step.

\begin{lemma}[Expectation step]\label[lemma]{lem:expectation-step}
  Let $Z_1,\ldots,Z_k \in \R^d$ be i.i.d. copies of a random variable $Z$ which has $\E Z = 0$ and $\E ZZ^\top = \Sigma$.
  If $r \geq 1000 (\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$, then $\E \max \, \pE \sum_{i=1}^k b_i \leq k/50$ where the maximum is taken over degree $2$ pseudodistributions on variables $b_1,\ldots,b_k,v_1,\ldots,v_d$ which satisfy $\cA = \{b_i^2 \leq 1, \|v\|^2 \leq 1, b_i (\iprod{Z,v} - r) \geq 0 \}$.
\end{lemma}


\begin{lemma}[Concentration step]\label[lemma]{lem:concentration-step}
  Let $Z_1,\ldots,Z_k \in \R^d$.
  Let $Z_1',\ldots,Z_k' \in \R^d$ be identical to $Z_1,\ldots,Z_k$ except for exactly one $i \in [k]$ with $Z_i \neq Z_i'$.
  Let $r > 0$.
  Let $\cA = \{b_i^2 \leq 1, \|v\|^2 \leq 1, b_i(\iprod{Z_i - \mu,v} - r) \geq 0\}$ and $\cA' = \{b_i^2 \leq 1, \|v\|^2 \leq 1, b_i(\iprod{Z_i' - \mu,v} - r) \geq 0 \}$.
  Then
  \[
  \Abs{ \max_{\pE \text{ satisfies } \cA} \pE \sum_{i=1}^k b_i - \max_{\pE \text{ satisfies }\cA'} \pE \sum_{i=1}^k b_i } \leq 1
  \]
  where the maximum is taken over degree-$2$ pseudodistributions.
\end{lemma}

\cref{lem:mu-is-certifiable} follows easily from \cref{lem:expectation-step,lem:concentration-step}.

\begin{proof}[Proof of \cref{lem:mu-is-certifiable}]
  Let
  \[
    f(Z_1,\ldots,Z_k) = \max_{\pE \text{ satisfies } \cA} \pE \sum_{i=1}^k b_i\mper
  \]
  For $r \geq 1000 (\sqrt{\Tr \Sigma/k} + \sqrt{\|\Sigma\|})$ from \cref{lem:expectation-step} we obtain that $\E f \leq k/50$.
  By the bounded differences inequality and \cref{lem:concentration-step}, we find
  \[
    \Pr_{Z_1,\ldots,Z_k} ( f(Z_1,\ldots,Z_k) - \E f(Z_1,\ldots,Z_k) > k/50 ) \leq \exp(-k/2000)\mper
  \]
  which proves the lemma.
\end{proof}

We turn to the proofs of \cref{lem:expectation-step,lem:concentration-step}.
To prove \cref{lem:expectation-step}, we use the following lemma, which is proved in \cref{sec:2-to-1-random} by standard empirical process theory.
It bounds the expected $2$-to-$1$ norm of a random matrix with i.i.d. rows.

%\begin{lemma}\label[lemma]{lem:2-to-1}
%  Let $Z$ be an $\R^d$-valued random variable with mean $\E Z = 0$ and covariance $\E ZZ^\top = \Sigma$.
%  Let $Z_1,\ldots,Z_k$ be iid copies of $Z$, and let $A \in \R^{k \times d}$ be the matrix whose rows are $\tfrac 1k Z_1,\ldots, \tfrac 1k Z_k$.
%  Then
%  \[
%  \E \|A\|_{2 \rightarrow 1} \leq 2 \sqrt{\frac{\Tr \Sigma}{k}} + \sqrt{\|\Sigma\|}
%  \]
%  where $\|\Sigma\|$ denotes the operator norm, or maximum eigenvalue, of $\Sigma$.
%\end{lemma}

Now we can prove \cref{lem:expectation-step}.
\begin{proof}[Proof of \cref{lem:expectation-step}]
  By centering the $Z_i$'s we may assume for convenience that $\mu = 0$.
  Fix a degree-$2$ pseudodistribution $\pE$ which satisfies $\{b_i^2 \leq 1, \|v\|^2 \leq 1, b_i (\iprod{Z_i,v} -r) \geq 0 \}$ with maximal $\pE \sum_{i=1}^k b_i$.
  We may assume that $\pE b_i \geq 0$, otherwise $\pE \sum_{i=1}^k b_i$ is increased by replacing $b_i$ with $0$, which still satisfies $b_i^2 \leq 1, b_i(\iprod{Z_i,v} -r) \geq 0$.
  And we may assume that $\pE b_i^2 = 1$, otherwise again $\pE \sum_{i=1}^k b_i$ is increased by replacing $b_i$ with $b_i/(\pE b_i^2)^{1/2}$.

  Since $\pE$ satisfies $b_i(\iprod{Z_i,v}-r) \geq 0$,
    \[
    \pE \sum_{i=1}^k b_i \leq \frac 1 r \cdot \pE \sum_{i=1}^k b_i \iprod{Z_i,v}\mper
    \]
    Because the left-hand side is nonnegative, so is the right-hand side.
    And thus it is only increased by replacing $v$ with $v / (\pE \|v\|^2)^{1/2}$, so we may assume $\pE \|v\|^2 = 1$.
    All in all,
    \[
      \max_{\substack{ \pE \text{ satisfies } \\ b_i^2 \leq 1 \\ \|v\|^2 \leq 1 \\ b_i (\iprod{Z_i,v} -r) \geq 0 }} \pE \sum_{i=1}^k b_i \leq \max_{\substack{\pE\|v\|^2 = 1 \\ \pE b_i^2 = 1}} \pE \sum_{i=1}^k b_i \iprod{Z_i,v}\mper
    \]
    The latter is exactly the SDP relaxation of the $2 \rightarrow 1$ norm of the matrix with rows $Z_i$.
    Hence the above is at most $2 \|A\|_{2 \rightarrow 1}$, where $A$ is the matrix with rows $Z_1,\ldots,Z_k$, by \cref{thm:sos-2-to-1}.
    Taking expectations on both sides and applying \cref{lem:2-to-1} completes the proof.
\end{proof}

It remains to prove \cref{lem:concentration-step}.

\begin{proof}[Proof of \cref{lem:concentration-step}]
  Without loss of generality, suppose that $Z_k \neq Z_k'$.
  By symmetry it will suffice to prove that
  \[
  \max_{\pE \text{ satisfies } \cA} \pE \sum_{i=1}^k b_i \leq \max_{\pE \text{ satisfies } \cA'} \pE \sum_{i=1}^k b_i + 1\mper
  \]
  Take any feasible solution $\pE$ to the left-hand side.
  Consider $\pE'$ defined by $\pE'p(b,v) = \pE p(b_1,\ldots,b_{k-1},0,v)$.
  Then $\pE'$ satisfies both $\cA$ and $\cA'$.
  Furthermore, $|\pE b_i| \leq (\pE b_i^2)^{1/2} \leq 1$, so $\pE' \sum_{i=1}^k b_i \geq \pE \sum_{i=1}^k b_i -1$.
\end{proof}


\subsection{SoS duality: \cref{lem:apply-duality}}

In this section we prove \cref{lem:apply-duality}.

\begin{proof}[Proof of \cref{lem:apply-duality}]
    Fix $\e > 0$.
    Let $\cA = \{b_i^2 \leq 1, b_i (\iprod{Z_i - \mu,v} -r) \geq 0, \|v\|^2 \leq 1\}$.
    By summing the constraints $b_i^2 \leq 1$ and $\|v\|^2 \leq 1$, we may assume that $\cA$ contains the inequality $\sum_{i=1}^k b_i^2 + \|v\|^2 \leq k+1$.
    Fix $\delta > 0$.
    Applying \cref{thm:duality} with $d=2$, either for every $\e > 0$ there is a degree $2$ SoS proof
    \[
    \cA \proves{2} (p+\delta) k - \sum_{i =1}^k b_i \geq -\e
    \]
    or there is a degree-$2$ pseudodistribution $\pE$ satisfying $\cA$ with $\pE \sum_{i=1}^k b_i \geq (p+\delta) k$.
    The latter is impossible by hypothesis, so for every $\e' > 0$ there is an SoS proof $\cA \proves{2} (p+\e') k - \sum_{i=1}^k b_i \geq 0$.

    Expanding the definition of SoS proof, there are SoS polynomials $\alpha_i,\beta_i,\gamma,\sigma$ such that
    \begin{align*}
    (p+\e') k - \sum_{i=1}^k b_i & = \sum_{i=1}^k \alpha_i(v,b) b_i (\iprod{Z_i-\mu,v}-r)
    + \sum_{i=1}^k \beta_i(v,b) (1-b_i^2)\\
    & + \gamma(v,b) (1-\|v\|^2)
    + \sigma(v,b)\mper
    \end{align*}
    such that all of $\alpha_i(v,b) b_i(\iprod{Z_i-\mu,v} - r), \beta_i(v,b) (1-b_i^2), \gamma(v,b)(1-\|v\|^2)$ have degree at most $2$.
    But then $\alpha_i,\beta_i,\gamma$ must be nonnegative constants (that is, polynomials of degree $0$) otherwise the degrees of these polynomials would be too high.
    So $\mu$ is a certifiable $(p+\e')$-th $r$-percentile.
\end{proof}


Finally, we establish that $\mu$ is \emph{nicely} certifiable.
In the sequel, $M$ should be thought of as $\Theta(\sqrt{\Tr \Sigma})$ and $r = \Theta(\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$, so $M/r \leq O(\sqrt{k})$.

\begin{lemma}\label[lemma]{lem:make-it-nice}
  Suppose that $Z_1,\ldots,Z_k,\mu \in \R^d$ and that $\mu$ is a certifiable $p$-th $r$-percentile of $Z_1,\ldots,Z_k$.
  Suppose also that only $qk$ vectors $Z_i$ have $\|Z_i - \mu \| \geq M$ for some $q \in [0,1]$.
  Then $\mu$ is a $(c, 4k/r )$-nicely certifiable $(p + q + 1/20)$-th percentile for $c = \min(1/r,1/M)/100$.
\end{lemma}




==> content/introduction <==
\section{Introduction}


==> content/sos-median.tex <==
\section{Main Algorithm and Analysis}
\label[section]{sec:main-alg}

Our algorithm employs a median-of-means scheme: first, the samples $X_1,\ldots,X_n$ are placed into $k = \Theta(\log 1/\delta)$ buckets at random, and the algorithm computes the empirical means $Z_1,\ldots,Z_k$ inside the buckets.
Then, the algorithm computes a certain median of the vectors $Z_1,\ldots,Z_k$.
The polynomial time algorithm for this median computation is the main technical contribution of this paper.
It is captured in the following lemma.

\begin{lemma}[\textsc{median-sdp}]\label[lemma]{lem:median-main}
  For every $k,d \in \N$ there is an algorithm \textsc{median-sdp} with running time $(kd)^{O(1)}$ such that for every $\R^d$-valued random variable $Z$ with $\E Z = \mu$ and $\E (Z-\mu)(Z-\mu)^\top = \Sigma$, given $k$ i.i.d. copies $Z_1,\ldots,Z_k$ of $Z$ \textsc{median-sdp} returns a vector $\hat{\mu}$ such that with probability at least $1-\exp(-k/100)$ over $Z_1,\ldots,Z_k$,
  \[
  \|\mu - \hat{\mu}\| \leq 64 \Paren{\sqrt{\frac{\Tr \Sigma}k} + \sqrt{\|\Sigma\|} }\mper
  \]
\end{lemma}

From \cref{lem:median-main} we can prove the main theorem.

\begin{proof}[Proof of \cref{thm:main}]
  Let $k = 100 \log(1/\delta)$.
  Without loss of generality, assume that $k$ divides $n$.
  Then let $Z_i$ be the average inside the $i$-th bucket:
  \[
    Z_i = \frac k n \sum_{j= in/k}^{(i+1)n/k} X_i\mper
  \]
  The vectors $Z_1,\ldots,Z_k$ are i.i.d. with mean $\E Z = \E X =\mu$ and covariance $\Sigma_Z = \tfrac kn \Sigma$.
  The output of our algorithm is the algorithm \textsc{median-sdp} of \cref{lem:median-main} on the vectors $Z_1,\ldots,Z_k$.
  With probability at least $1-\delta$ (by the definition of $k$), then the resulting estimator $\hat{\mu}$ satisfies
  \[
    \|\mu - \hat{\mu}\| \leq 64 \Paren{\sqrt{\frac{\Tr \Sigma_Z}k} + \sqrt{\|\Sigma_Z\|} } \leq 640 \Paren{\sqrt{\frac{\Tr \Sigma}{n}} + \sqrt{\frac{\|\Sigma\| \log(1/\delta) }{n}}}\mper\qedhere
  \]
\end{proof}

The remainder of the paper is devoted to the algorithm \textsc{median-sdp} and the proof of \cref{lem:median-main}.

\subsection{The median polynomial program}

We recall the setting: there is a $d$-dimensional random vector $Z$ with finite mean $\mu$ and covariance $\Sigma$ (we drop the subscript $Z$ on $\Sigma$ from the previous subsection, since now the random variable $X$ has left the picture).
Given $k$ i.i.d. samples $Z_1,\ldots,Z_k$ from $Z$, the goal is to find a vector $\hat{\mu}$ such that $\|\mu - \hat{\mu}\| \leq 64 (\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$, with probability at least $1- \exp(-k/100)$.
The starting point of \textsc{median-sdp} is a semidefinite relaxation of the following optimization problem.

\begin{definition}[Median Polynomial Program]
  Let $Z_1,\ldots,Z_k \in \R^d$.
  The median polynomial program is:
  \begin{align*}
  & \min_{x \in \R^d} \max_{v \in \R^d} \|v\|^2 \\
  \text{such that } \quad & b_i^2 = b_i \text{ for $i \leq k$}\\
  & \sum_{i \leq k} b_i = \frac k2 \\
  & b_i \iprod{Z_i - x, v} \geq b_i \cdot \|v\|^2 \mper
  \end{align*}
  Notice that the constraints $b_i^2 = b_i$ are solved only by $b_i \in \{0,1\}$.
  By rearranging the constraints one may see that feasible solutions are pairs $b,v$ where $b$ is the indicator of $B \subseteq [k]$ with $|B| \geq k/2$ such that for every $i \in B$ it holds that $\|Z_i - (x+2v)\| \leq \|Z_i - x\|$.
\end{definition}

Implicit in the work of Lugosi and Mendelson \cite{LM18} is the following lemma:
\begin{lemma}[\cite{LM18}, implicit]\label[lemma]{lem:lm18-main}
  With probability at least $1-\exp(-k/C)$, any minimizer $x^*$ of the median polynomial program satisfies $\|x^* - \mu\| \leq C(\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$ for some universal constant $C$.
\end{lemma}
Thus, an efficient algorithm to find a minimizer of the median polynomial program would solve our mean estimation problem.
Unfortunately, there is no clear algorithm to solve the median polynomial program.
Instead, our algorithm will solve a semidefinite relaxation of it.
Our main technical lemma will be an analogue of \cref{lem:lm18-main} for our relaxation.

In the remainder of this section we describe \textsc{median-sdp}, which is our semidefinite relaxation, and provide its main analysis.
First we need some background.

\subsection{\textsc{median-sdp}}

% We need just one more definition before setting up \textsc{median-sdp}.

%\begin{definition}\label[definition]{def:extends}
%  Let $\pE_1$ be a degree $t$ pseudoexpectation on variables $x=x_1,\ldots,x_n$ and $\pE_2$ be of degree $t' \geq t$ on variables $x_1,\ldots,x_n,y_1,\ldots,y_m$.
%  We say $\pE_2$ extends $\pE_1$ if $\pE_1 p(x) = \pE_2 p(x)$ for all $p \in \R[x_1,\ldots,x_n]_{\leq t}$.
%\end{definition}

\begin{definition}[\textsc{median-sdp}]\label[definition]{def:median-sdp}
  Let $Z_1,\ldots,Z_k \in \R^d$.
  In the following, $\pE$ is a pseudodistribution on variables $x_1,\ldots,x_d$ and $\pE'$ is on $x'_1,\ldots,x'_d,v_1,\ldots,v_d,b_1,\ldots,b_k$.
  (Notice that this is the same set of variables as in the median polynomial program.)
  $\pE,\pE'$ are both of degree $4$.
  The \textsc{median-sdp} is:
  \begin{align}
  \textsc{median-sdp}(Z_1,\ldots,Z_k) =  & \min_{\pE} \max_{ \pE'} \, \, \pE' \|v\|^2 \text{ such that } \nonumber \\
  & \text{ $\pE'$ satisfies } b_i^2 - b_i = 0 \text{ for all $i \leq k$} \\
  & \text{ $\pE'$ satisfies } \sum_{i \leq k} b_i - \frac k2 = 0 \\
  & \pE' b_i \iprod{Z_i - x',v} \geq \pE' b_i \|v\|^2 \text{ for all $i \leq k$} \\
  & \pE' \pE \|x-x'\|^2 = 0\mper
  \end{align}
\end{definition}

Our main lemma on \textsc{median-sdp}, and the main technical lemma of this paper, is the following.
\begin{lemma}\label[lemma]{lem:med-sdp-main}
  Suppose $Z_1,\ldots,Z_k$ are i.i.d. with mean $\mu$ and covariance $\Sigma$.
  Let $\pE^*$ be the optimizer of \textsc{median-sdp} on $Z_1,\ldots,Z_k$.
  With probability at least $1 - \exp(-k/100)$, the vector $\pE^* x$ (whose $i$-th entry is $\pE^* x_i$) has $\|\pE^* x - \mu\| \leq 64 (\sqrt{\Tr \Sigma / k} +\sqrt{\|\Sigma\|})$.
\end{lemma}
In \cref{sec:explicit-sdp}, we design more explicit semidefinite programs whose solutions are the pseudodistributions $\pE$ and $\pE'$ of \textsc{median-sdp}.
It then becomes clear that the function $f(\pE) = \max_{\pE'} \pE' \|v\|^2$ is convex in $\pE$, and can be evaluated by solving a semidefinite program; \textsc{median-sdp} is therefore solvable by the Ellipsoid algorithm.
Thus, along with the running time analysis in \cref{sec:explicit-sdp}, \cref{lem:med-sdp-main} implies \cref{lem:median-main}.
We expect that solving the optimization problem with a more tailor-made algorithm (using a first or second order descent method, for instance) will lead to much faster running times, but this requires a more sophisticated analysis.

In the remainder of this section, we prove \cref{lem:med-sdp-main} from sublemmas, which we then prove in subsequent sections.
The first lemma bounds the inner variational problem in \textsc{median-sdp} (the maximization over $\pE'$) in the case that $\pE p(x) = p(\mu)$ for all $p$.
We prove it in \cref{sec:sdp-cert}.

\begin{lemma}\label[lemma]{lem:mean-cert}
  Let $Z_1,\ldots,Z_k$ in $\R^d$ be i.i.d. with mean $\mu$ and covariance $\Sigma$.
  Let $\pE$ be the degree $4$ pseudoexpectation in variables $x_1,\ldots,x_d$ such that $\pE p(x) = p(\mu)$.
  With probability at least $1-\exp(-k/100)$,
  \[
    \max_{\pE'} \pE' \|v\|^2 \leq 60 \Paren{\frac{\Tr \Sigma}{k} +\|\Sigma\|}\mcom
  \]
  where the maximization is over $\pE'$ satisfying the constraints of \textsc{median-sdp}.
\end{lemma}

The second lemma is a pseudoexpectation version of the observation that for every pair of vectors $x_0,x_1 \in \R^d$, either $\|x_0 - Z_i\| \geq \|x_1 - Z_i\|$ for at least half of the vectors $Z_i$, or $\|x_1- Z_i\| \geq \|x_0 - Z_i\|$ for at least half of the $Z_i$'s.


\begin{lemma}\label[lemma]{lem:one-must-defeat}
  Suppose $\pE_0$ is a degree $4$ pseudodistribution on variables $x_1,\ldots,x_d,v_1,\ldots,v_d$.
  Let $Z_1,\ldots,Z_k \in \R^d$.
  Then at least one of the following holds.
  \begin{enumerate}
    \item $\pE_0$ can be extended to $\pE'$ which is feasible for \textsc{median-sdp}.
    \item Let $\pE_1 p(x,v) = \pE p(x+2v,-v)$. Then $\pE_1$ can be extended to $\pE'$ which is feasible for \textsc{median-sdp}.
  \end{enumerate}
\end{lemma}

We prove \cref{lem:one-must-defeat} in \cref{sec:one-must-defeat}.
We also need an elementary fact.

\begin{fact}\label[fact]{fact:2-norm}
  Suppose that $\pE$ is a degree $2$ pseudoexpectation on $x$, and that $\mu \in \R^d$.
  Then $\| \pE x - \mu\|^2 \leq \pE \|x - \mu\|^2$.
\end{fact}
\begin{proof}
  Since $\| x - \mu\|^2 = \sum_{i \leq d} (x_i - \mu_i)^2$, this follows from the more general statement that $\pE p(x)^2 \geq (\pE p(x))^2$.
  This in turn follows from $\pE (p(x) - \pE p(x))^2 \geq 0$, since
  \[
  0 \leq \pE( p(x) - \pE p(x))^2 = \pE p(x)^2 - (\pE p(x))^2\mper \qedhere
  \]
\end{proof}

Now we can prove \cref{lem:med-sdp-main}.
\begin{proof}[Proof of \cref{lem:med-sdp-main}]
  Suppose that the event of \cref{lem:mean-cert} occurs.
  Let $(\pE,\pE')$ be the optimizers of \textsc{median-sdp}.
  Since $\pE_\mu$ given by $\pE p(x) = p(\mu)$, is also a feasible solution to \textsc{median-sdp}, by \cref{lem:mean-cert} we know that $\pE' \|v\|^2 \leq 64 \Paren{\frac{\Tr \Sigma}{k} +\|\Sigma\|}$.

  Consider the pseudodistribution $\pE_0$ on $x_1,\ldots,x_d,v_1,\ldots,v_d$ given by $\pE_0 p(x,v) = \pE p(x, \tfrac 12 (\mu - x))$.
  Suppose that the first case of \cref{lem:one-must-defeat} applies to it, so there exists a pseudodistribution $\pE_0'$ extending $\pE_0$ and feasible for \textsc{median-sdp}.
  Then $\pE_0' \|v\|^2 \leq \pE' \|v\|^2 \leq 64 \Paren{\frac{\Tr \Sigma}{k} +\|\Sigma\|}$.
  But since $\pE_0' \|v\|^2 = \pE_0 \|v\|^2 = \tfrac 14 \pE \|\mu - x\|^2$, we are done by \cref{fact:2-norm}.
  If the second case of \cref{lem:one-must-defeat} applies, then notice that $\pE_1 p(x,v) = \pE_0(\mu,\tfrac 12 (x - \mu))$, and the same argument applies using \cref{lem:mean-cert}.
\end{proof}


\subsection{Proof of \cref{lem:one-must-defeat}}
\label[section]{sec:one-must-defeat}
In this section we prove \cref{lem:one-must-defeat}.

\begin{proof}[Proof of \cref{lem:one-must-defeat}]
  In both cases we will construct the solution by taking $\pE' p(x,v,b) = \pE p(x,v,\bb)$ for some $\bb \in \{0,1\}^k$ where either $\pE = \pE_0$ or $\pE = \pE_1$.
  That is, $\pE'$ will look like an integral solution with respect to the $b$ variables.
  Consider the numbers $a_i = \pE_0 \iprod{Z_i -x,v} - \pE_0 \|v\|^2$.
  If at least half of them satisfy $a_i \geq 0$, then let $\bb$ be the indicator of a set of exactly $k/2$ indices with $a_i \geq 0$.

  Otherwise, consider $a_i' = \pE_1 \iprod{Z_i -x,v} - \pE_1 \|v\|^2$.
  We have
  \begin{align*}
  \pE_1 \iprod{Z_i-x,v} - \pE_1 \|v\|^2 & = \pE_0 \iprod{Z_i - x - 2v,-v} - \pE_0 \|v\|^2\\
  & = 2 \pE_0 \|v\|^2 - \pE_0 \iprod{Z_i -x,v} - \pE_0 \|v\|^2\mper
  \end{align*}
  Thus if $a_i < 0$ then $a_i' \geq 0$.
  So, choose $\bb$ to be the indicator of a set of exactly $k/2$ indices where $a_i' \geq 0$.
\end{proof}



\section{SDP certificates for the median}
\label[section]{sec:sdp-cert}
In this section we prove \cref{lem:mean-cert}.
The proof has two main steps, an expectation step and a concentration step.
Both steps involve another semidefinite program, used only for purposes of analysis, which we call \textsc{threshold-sdp}.
This SDP is a relaxation of the following problem: given vectors $Z_1,\ldots,Z_k$, find $v$ on the unit sphere maximizing the number of $i \in [k]$ such that $\iprod{Z_i,v} \geq r$ for some threshold $r > 0$.

\begin{definition}[\textsc{threshold-sdp}]
  Let $Z_1,\ldots,Z_k \in \R^d$.
  For a parameter $r > 0$, let
  \begin{align*}
  \textsc{threshold-sdp}_r(Z_1,\ldots,Z_k) = & \max_{C > 0} \, C \, \text{ such that there exists $\pE$ with }\\
  & \text{ $\pE$ satisfies } b_i^2 - b_i = 0 \\
  & \text{ $\pE$ satisfies } \sum_{i \leq k} b_i \geq C \\
  & \pE \|v\|^2 = 1 \\
  & \pE b_i \iprod{Z_i,v} \geq \pE b_i \|v\|^2 \cdot r
  \end{align*}
  where $\pE$ ranges over degree $4$ pseudodistributions in variables $v_1,\ldots,v_d, b_1,\ldots,b_k$.
\end{definition}


\begin{lemma}[Expectation step]\label[lemma]{lem:expectation-step}
  Let $Z_1,\ldots,Z_k \in \R^d$ be i.i.d. copies of a random variable $Z$ which has $\E Z = 0$ and $\E ZZ^\top = \Sigma$.
  If $r \geq 24 (\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$, then $\E \textsc{threshold-sdp}_r(Z_1,\ldots,Z_k) \leq k/4$.
\end{lemma}


\begin{lemma}[Concentration step] \label[lemma]{lem:concentration-step}
  For any $r > 0$ and any set of vectors $Z_1,\ldots,Z_k \in \R^d$ and any other vector $Z_i' \in \R^d$,
  \begin{align*}
    |\textsc{threshold-sdp}_r & (Z_1,\ldots,Z_k) -\\
    & \textsc{threshold-sdp}_r(Z_1,\ldots,Z_{i-1},Z_i',Z_{i+1},\ldots,Z_k) | \leq 1\mper
  \end{align*}
\end{lemma}

Now we can prove \cref{lem:mean-cert}.

\begin{proof}[Proof of \cref{lem:mean-cert}]
  Taken together, \cref{lem:expectation-step} and \cref{lem:concentration-step} imply via the bounded differences inequality that with probability at least $1- \exp(-k/100)$ it holds that $\textsc{threshold-sdp}_r(Z_1-\mu,\ldots,Z_k-\mu) \leq k/3$ so long as $r \geq 24 (\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$.
  Now, let $\pE$ on $x_1,\ldots,x_d$ be given by $\pE p(x) = p(\mu)$, and suppose that there were $\pE'$ extending $\pE$ and feasible for \textsc{median-sdp} with $\pE'\|v\|^2 > 60 (\Tr \Sigma/k + \|\Sigma\|)$.
  Let $\pE''$ be a renormalization of $\pE'$, where 
  \[
    \pE''p(x,v,b) = \pE'p\Paren{x,\tfrac {v}{(\pE'\|v\|^2)^{1/2}}, b}\mper
  \]

  We claim that $\pE''$ satisfies the constraints of $\textsc{threshold-sdp}_r(Z_1-\mu,\ldots,Z_k-\mu)$, with $r = (\pE' \|v\|^2)^{1/2}$ and $C = k/2$.
  The only nontrivial constraint to check is $\pE'' b_i\iprod{Z_i,v} \geq r \pE b_i \|v\|^2$.
  But since $\pE'$ satisfies \textsc{median-sdp},
  \[
    \pE'' b_i\iprod{Z_i-\mu,v} = \frac {\pE' b_i \iprod{Z_i-\mu,v}}{\sqrt{\pE \|v\|^2}} \geq \frac 1r \pE' b_i \|v\|^2 = r \pE'' b_i \|v\|^2\mper
  \]
  Since $C = k/2 > k/3$, this means that we must have $r \leq 24 (\sqrt{\Tr \Sigma / k} + \sqrt{\|\Sigma\|})$.
\end{proof}


\subsection{Expectation step}
In this section we prove \cref{lem:expectation-step}.
The main tools will be a variant of Grothendieck's inequality and a bound on the expected $2$-to-$1$ norm of a random matrix.
We start with a definition.

Now we can prove \cref{lem:expectation-step}.
\begin{proof}[Proof of \cref{lem:expectation-step}]
  Let $\pE$ be a feasible solution to \textsc{threshold-sdp}.
  Then
  \[
    C \cdot \pE \|v\|^2  \leq \pE \sum_{i \leq k} b_i \|v\|^2 \leq \frac 1r \pE \sum_{i \leq k} b_i \iprod{Z_i,v}
  \]
  using that $\pE$ satisfies $\sum_{i \leq k} b_i \geq C$ and $\pE b_i \iprod{Z_i,v} \geq \pE b_i \|v\|^2 r$.
  Let $\sigma_i = 2b_i -1$ and notice that if $b_i^2 - b_i = 0$ then $\sigma_i^2 - 1 = 0$.
  We rearrange the right-hand side of the above to
  \[
    \frac 1r \pE \sum_{i \leq k} b_i \iprod{Z_i,v} = \frac 1r \Paren{ \frac 12 \pE \sum_{i \leq k} \sigma_i \iprod{Z_i,v} + \frac 12 \pE \sum_{i \leq k} \iprod{Z_i,v} }\mper
  \]
  By \cref{lem:sos-2-to-1}, we have $\pE \sum_{i \leq k} \sigma_i \iprod{Z_i,v} \leq 2 \|A\|_{2 \rightarrow 1}$, where the rows of $A$ are the vectors $Z_1,\ldots,Z_k$.
  Also,
  \[
  \pE \sum_{i \leq k} \iprod{Z_i,v} \leq \|\pE v\| \cdot \Norm{\sum_{i \leq k} Z_i} \leq \Norm{\sum_{i \leq k} Z_i}\mper
  \]
  So in the end we obtained
  \[
  \E c^*(Z_1,\ldots,Z_k) \leq \frac 1r \Paren{ \E \|A\|_{2 \rightarrow 1} + \E \Norm{ \sum_{i \leq k} Z_i }} \leq \frac 4 r \Paren{ \sqrt{k \Tr \Sigma} + k \sqrt{\|\Sigma\|}}\mper
  \]
  (Here we used \cref{lem:2-to-1} to bound $\E \|A\|_{2 \rightarrow 1}$.)
  This proves the lemma.
\end{proof}

\subsection{Concentration step}

We prove \cref{lem:concentration-step}.

\begin{proof}[Proof of \cref{lem:concentration-step}]
  By symmetry, without loss of generality we assume $i=k$.
  Let $\pE$ be a feasible solution to $\textsc{threshold-sdp}(Z_1,\ldots,Z_k)$ with objective value $C$.
  We claim that $\pE$ satisfies $\sum_{i \leq k-1} b_i \geq C -1$.
  To see this first note that for any $p$ with $\deg p^2 \leq 2$,
  \[
  \pE p^2(1-b_i) = \pE p^2(1-b_i)^2 \geq 0
  \]
  because $\pE$ satisfies $b_i^2 -b_i=0$.
  So,
  \[
  \pE \Brac{p^2 \cdot \Paren{\sum_{i \leq k-1 } b_i - (C-1)}} = \pE \Brac{ p^2 \sum_{i \leq k} b_i - C} + \pE \Brac{ p^2  (1 - b_k) } \geq 0\mper
  \]
  Thus, $\pE$ restricted to $v,b_1,\ldots,b_{k-1}$ is feasible for $\textsc{threshold-sdp}(Z_1,\ldots,Z_{k-1})$ with objective value $C-1$, which means
  \[
  \textsc{threshold-sdp}(Z_1,\ldots,Z_k) \leq \textsc{threshold-sdp}(Z_1,\ldots,Z_{k-1}) +1\mper
  \]
  However, any feasible solution $\pE$ for $\textsc{threshold-sdp}(Z_1,\ldots,Z_{k-1})$ can be extended to a feasible solution to $\textsc{threshold-sdp}(Z_1,\ldots,Z_k')$ by adding the variable $b_k$ but setting it to $0$.
  So
  \[
    \textsc{threshold-sdp}(Z_1,\ldots,Z_{k-1}) \leq \textsc{threshold-sdp}(Z_1,\ldots,Z_{k}')
  \]
  which finishes the proof.
\end{proof}

\iffalse


\subsection{OLD OLD OLD}

For notational convenience, we take a \emph{pseudoexpectation} point of view on the semidefinite program.

\begin{definition}[Pseudoexpectation]
  A pseudoexpectation of degree $t \in \N$ on variables $x_1,\ldots,x_n$ is a functional $\pE \, : \, \R[x_1,\ldots,x_n]_{\leq t} \rightarrow \R$ on polynomials of degree at most $t$ which satisfies
  \begin{enumerate}
  \item (Normalization) $\pE[1] = 1$
  \item (Linearity) $\pE[ap(x) + bq(x)] = a\pE[p(x)] + b\pE[q(x)]$ for all $p,q \in \R[x_1,\ldots,x_n]_{\leq t}$ and $a,b \in \R$.
  \item (Positivity) $\pE[p(x)^2] \geq 0$ for all $p \in \R[x_1,\ldots,x_n]_{\leq t/2}$.
  \end{enumerate}
\end{definition}

\begin{definition}\label[definition]{def:extends}
  If $\pE$ is a degree $t$ pseudoexpectation on $x=x_1,\ldots,x_n$ and $\pE'$ is a degree $d$ pseudoexpectation on $x_1,\ldots,x_n, y_1,\ldots,y_m$ then $\pE'$ \emph{extends} $\pE$ if $\pE[p(x)] = \pE'[p(x)]$ for every $p \in \R[x]_{\leq t}$.
\end{definition}

\begin{definition}\label[definition]{def:satisfies}
  A degree $t$ pseudoexpectation $\pE$ on $x=x_1,\ldots,x_n$ \emph{satisfies} $p(x) = 0$ if $\pE[p(x)q(x)] = 0$ for all $q$ such that $\deg(p\cdot q) \leq t$.
  It satisfies $p(x) \geq 0$ if $\pE[p(x) q(x)^2] \geq 0$ for all $q$ such that $\deg (p \cdot q^2) \leq t$.
\end{definition}


\begin{definition}[Median SDP]
\label[definition]{def:med-sdp}
  Let $Z_1,\ldots,Z_k \in \R^d$.
  \textsc{median-sdp} is:
  \begin{align*}
    & \min_{\substack{\pE \text{ on } x_1,\ldots,x_d \\ \deg \pE = 4}} \, \, \max_{\substack{\pE' \text{ on } \\ x_1,\ldots,x_d \\ y_1,\ldots, y_d \\ b_1,\ldots,b_k \\ \text{ extends } \pE}}  \pE\nolimits' \|x-y\|^2\\
  \text{such that } \quad & \pE\nolimits' \text{ satisfies } b_i^2 - b_i = 0 \text{ for } i \leq k\\
  & \pE\nolimits' \text{ satisfies } b_i ( \|Z_i - y\|^2 - \|Z_i - x\|^2) \geq 0 \text{ for } i \leq k\mper
  \end{align*}
\end{definition}

\paragraph{Relation to semidefinite programming}
\Snote{TODO:write this}


Our main technical lemma is the following.
\Snote{TODO:improve flavor text}

\begin{lemma}\label[lemma]{lem:cert-main}
  Let $Z_1,\ldots,Z_k$ be i.i.d. copies of a random variable $Z$ on $\R^d$ with $\E Z = \mu$ and $\E(Z-\mu)(Z -\mu)^\top = \Sigma$.
  With probability at least $1-\exp(-k/100)$,
  \[
  \max_{\pE} \pE \|\mu- y\|^2 \leq 1000\Paren{\frac{\Tr \Sigma}k + \|\Sigma\|}\mcom
  \]
  where the maximization is over degree $4$ pseudoexpectations $\pE$ on variables $y_1,\ldots,y_d,b_1,\ldots,b_k$ which satisfy $b_i^2 - b_i = 0$ for $i \leq k$ and $b_i(\|Z_i - y\|^2 - \|Z_i - x\|^2) \geq 0$ for $i \leq k$.
\end{lemma}

We also need the following lemma.

\begin{lemma}\label[lemma]{lem:one-must-defeat}
  Let $\pE_0, \pE_1$ be pseudoexpectations q   on var
\end{lemma}

The next lemma then follows; it is our main tool to prove the main theorem.

\begin{lemma}\label[lemma]{lem:cert-implies}
  Let $Z_1,\ldots,Z_k$ be i.i.d. copies of a random variable $Z$ on $\R^d$ with $\E Z = \mu$ and $\E(Z-\mu)(Z -\mu)^\top = \Sigma$.
  Let $\pE_*$ be the minimizer of the median SDP (\cref{def:med-sdp}) on $Z_1,\ldots,Z_k$.
  Then $\|\pE_* x - \mu \| \leq 100 \sqrt{\Tr \Sigma/ k} + 100\sqrt{\|\Sigma\|}$ with probability at least $1-\exp(-k/100)$.
\end{lemma}
\begin{proof}
  Let $r^2 = 1000\Paren{\frac{\Tr \Sigma}k + \|\Sigma\|}$.
  Suppose the event described in \cref{lem:cert-main} occurs.
  Then since $\pE_*$ is the minimizer, we know $\max_{\pE' \text{ extends } \pE_*} \pE'\|x-y\|^2 \leq r^2$.


\end{proof}


\begin{theorem}
  L
\end{theorem}





\section{Graveyard}
For such $Y$, we employ the following notation for its blocks:
\[
Y =
\left (
\begin{matrix}
  1 & Y^{1,X} & Y^{1,V} & Y^{1,B} & Y^{1, \iprod{x,v}}\\
  (Y^{1,X})^\top & X & Y^{X,V} & Y^{X,B} & Y^{X,\iprod{x,v}}\\
  (Y^{1,V})^\top & (Y^{X,V})^\top & V & Y^{V,B} & Y^{V,\iprod{x,v}} \\
  (Y^{1,B})^\top & (Y^{X,B})^\top & (Y^{V,B})^\top & B & Y^{B,\iprod{x,v}}\\
  (Y^{1,\iprod{x,v}})^\top & (Y^{X,\iprod{x,v}})^\top & (Y^{V,\iprod{x,v}})^\top & (Y^{B,\iprod{x,v}})^\top & Y^{\iprod{x,v}^2}
\end{matrix}
\right )\mper
\]
Here, $V \in \R^{d \times d}$ and $B \in \R^{k \times k}$ and $Y^{\iprod{x,v}^2} \in \R$, and the $1$ in the upper-left corner is the $1 \times 1$ identity matrix; the off-diagonal blocks have the appropriate dimensions.
Also, $Y^{1,X} = x^\top$.

\begin{definition}[Median SDP]
  Let $Z_1,\ldots,Z_k \in \R^d$.
  The median SDP is:
  \begin{align*}
    & \min_{\substack{X_0 \in \R^{(d+1) \times (d+1)}\\ X \succeq 0}} \, \, \max_{Y \text{ extends } X} \, r\\
  \text{such that } \quad & B_{ii} \leq 1 \text{ for $i \leq k$}\\
  & \Tr B = \frac k2 \\
  & \Tr V = 1 \\
  & \iprod{Z_i, Y^{VB}_i} - Y^{B,\iprod{x,v}}_i \geq B_{ii} r \text{ for $i \leq k$}\mper
  \end{align*}
\end{definition}

\paragraph{Functional Notation for SDP Solutions}
We introduce alternative notation for solutions to the median SDP, avoiding the block-matrix notation in the preceding definitions.
We identify any $Y \in \R^{(2d+k+2) \times (2d+k+2)}$ (as in \cref{def:extends}) with a linear functional $\bY \, : \, \cP \rightarrow \R$, where $\cP$ is a subspace of the vector space of polynomials in variables $x_1,\ldots,x_d, v_1,\ldots,v_d,$ and $b_1,\ldots,b_k$ given by
\[
\cP = \Span \left \{ p(x,v,b)q(x,v,b)  \, : \, p,q \in \Span \{ 1, x_1,\ldots,x_d,v_1,\ldots,v_d,b_1,\ldots,b_k, \iprod{x,v} \} \right \}\mper
\]
That is, $\cP$ contains all polynomials of degree at most $2$ in the variables $x,v,b,\iprod{x,v}$ (and hence some degree $3$ and $4$ polynomials in $x,v,b$).
The operator $\bY$ is given by
\[
\bY[p(x,v,b)] = \iprod{Y,M} = \Tr Y M^\top
\]
where $M \in \R^{(2d+k+2) \times (2d+k+2)}$ is any matrix such that $p(x,v,b) = (1,x,v,b,\iprod{x,v})^\top M (1,x,v,b,\iprod{x,v})$.





\begin{remark}[Relation to Sum of Squares Method]
\Snote{TODO}
\end{remark}



\begin{lemma}\label[lemma]{lem:one-must-defeat}
  Let $Z_1,\ldots,Z_k \in \R^d$.
  Let $Y_0 \in \R^{(2d+2) \times (2d+2)}$ be any PSD matrix with blocks
  \[
  Y_0 =
  \left (
  \begin{matrix}
    1 & Y_0^{1,X} & Y_0^{1,V}  \\
    (Y_0^{1,X})^\top & X & Y_0^{X,V} \\
    (Y_0^{1,V})^\top & (Y_0^{X,V})^\top & V \\
    (Y_0^{1,\iprod{x,v}})^\top & 
  \end{matrix}
  \right )
  \]
  where $\Tr V = 1$.
  Then either $Y_0$ can be extended to a PSD matrix $Y \in \R^{(2d+k+2) \times (2d +k+2)}$ which is feasible for \textsc{median-sdp} (\cref{def:med-sdp}) and having objective value $r$, or the following matrix $Y_0'$ can be:
  \[
  Y_0' =
  \left (
  \begin{matrix}
    1 & Y_0^{1,X} & - Y_0^{1,V}  \\
    (Y_0^{1,X'})^\top & X' & -Y_0^{X,V} \\
    (-Y_0^{1,V})^\top & (-Y_0^{X,V})^\top & V
  \end{matrix}
  \right )
  \]
  where $X' = X + 4 r^2 V + 2r Y_0^{X,V} + 2r (Y_0^{X,V})^\top$ and $Y_0^{1,X'} = Y_0^{1,X} + 2rY_0^{1,V}$.
\end{lemma}
As some intuition, consider the meaning of \cref{lem:one-must-defeat} in the case that that $Y_0$ is an integral solution $Y_0 = y_0y_0^\top$ where $Y = (1,x,v)$ for some $x,v \in \R^d$ with $\|v\|=1$.
If we think also of $B = bb^\top$ as an integral solution $b \in \{0,1\}^k$, the lemma simply says that either $\|Z_i - x\|^2 \leq \|Z_i - (x+2v)\|^2$ for at least $k/2$ vectors $Z_i$, or vice versa.

To see this, observe that in this integral case $Y_0'$ corresponds to the integral solution $(y_0')(y_0')^\top = (1,x+ 2r \cdot v, -v)$.
The statement of the lemma then says that either there are $k/2$ vectors $Z_i$ such that $\iprod{Z_i -x,v} \geq r$, or there are $k/2$ vectors $Z_i$ such that $\iprod{Z_i-x-2rv,-v} \geq r$.
This we can see because $\iprod{Z_i -x - 2rv, -v} = 2r \|v\|^2 - \iprod{Z_i-x,v} = 2r-\iprod{Z_i-x,v}$, which is at least $r$ if $\iprod{Z_i-x,v} \leq r$.

\begin{proof}[Proof of \cref{lem:one-must-defeat}]
  For each $i$, define $a_i = \Tr X - 2 \iprod{Z_i, Y_0^{1,X}} + \|Z_i\|^2$.
  (This plays the role of $\|Z_i -x\|^2$ from the integral case.)
  Define $a_i' = \Tr X' - 2 \iprod{Z_i, Y_0^{1,X'}} + \|Z_i\|^2$.

  Suppose that $a_i \geq a_i$ for at least $k/2$ indices $i \in [k]$.
  Then let $b \in \{0,1\}^k$ be the indicator vector of those indices.
  Define $B = bb^\top$ and $Y^{1,B} = b$.
  Then let $Y^{X,B} = (Y^{1,X})b^\top$ and similarly for $Y^{V,B}$.
  Then if $B_{ii} = b_i^2 = 1$, we have $Y_i^{VB} = Y^{1,V}$.

 
\end{proof}




\section{Main Algorithm and Analysis -- OLD}

To state our main algorithm we need to define a convex relaxation of a high-dimensional median.

\begin{definition}\label[definition]{def:extends}
  Let $\pE$ be a degree $t$ pseudodistribution on variables $x = x_1,\ldots,x_n$, and let $\pE'$ be a degree $t$ pseudodistribution on variables $x = x_1,\ldots,x_n$ and $y = y_1,\ldots,y_m$.
  We say $\pE'$ extends $\pE$ if $\pE p(x) = \pE' p(x)$ for every $p \in \R[x_1,\ldots,x_n]_{\leq d}$.
\end{definition}

\begin{definition}\label[definition]{def:median-poly}
  For vectors $Z_1,\ldots,Z_k \in \R^d$, let $\cA(Z_1,\ldots,Z_k)$ be the following system of polynomials in variables $x = x_1,\ldots,x_d$ and $y = y_1,\ldots,y_d$ and $b = b_1,\ldots,b_k$.
  \begin{align*}
    & b_i^2 = b_i \text{ for $i \leq k$}\\
    & b_i \|Z_i - y\|^2  \geq b_i \|Z_i - x\|^2 \text{ for $i \leq k$}\\
    & \sum_{i \leq k} b_i  \geq \frac k2\mper
  \end{align*}
\end{definition}

\begin{definition}\label[definition]{def:sos-median}
  For vectors $Z_1,\ldots,Z_k \in \R^d$, the \emph{SoS Median} is the following variational problem.
  \[
    \arg \min_{\pE} \max_{\pE'} \pE\nolimits' \|x - y\|^2
  \]
  where $\pE$ ranges over all degree $2$ pseudodistributions on variables $x = x_1,\ldots,x_d$ and $\pE'$ ranges over degree $4$ pseudodistributions on variables $x, y = y_1,\ldots,y_d$, and $b = b_1,\ldots,b_k$ which extend $\pE$ and satisfy $\cA(Z_1,\ldots,Z_k)$.
\end{definition}

\begin{algorithm}{Robust Mean Estimation}
\begin{algorithmic}[1]
\Function{EstimateMean}{$\delta,X_1,\ldots,X_n$}
\State Let $k = 32 \log \tfrac 1 \delta$. For $i \leq k$, let $Z_i = \tfrac 1k \sum_{k(i-1) \leq j < k} X_j$.
\State \textbf{return} \textsc{SoSMedian}$(Z_1,\ldots,Z_k)$.
\EndFunction
\Function{SoSMedian}{$Z_1,\ldots,Z_k$}
\State Solve the saddle point problem \cref{def:sos-median}, obtaining a pseudodistribution $\pE$ on variables $x = x_1,\ldots,x_d$.
\State \textbf{return} $\pE x$
\EndFunction
\end{algorithmic}
\label[algorithm]{alg:estimate-mean}
\end{algorithm}

Our main theorem follows from the following lemmas.

\begin{lemma}\label[lemma]{lem:sos-med-1}
  Let $Z_1,\ldots,Z_k \in \R^d$.
  For every vector $z \in \R^d$, the output $x$ of \textsc{SoSMedian}$(Z_1,\ldots,Z_k)$ satisfies
  \[
  \|x - z\|^2 \leq \max_{\substack{\pE \text{ satisfies }\\ \cB(z,Z_1,\ldots,Z_k)}} \pE \|z - y\|^2
  \]
  where $\pE$ is degree $4$ and $\cB(z,Z_1,\ldots,Z_k)$ is the following system of polynomials:
  \begin{align*}
    & b_i^2 = b_i \text{ for $i \leq k$}\\
    & b_i \|Z_i - y\|^2  \geq b_i \|Z_i - z\|^2 \text{ for $i \leq k$}\\
    & \sum_{i \leq k} b_i  \geq \frac k2
  \end{align*}
  That is $\cB(z,Z_1,\ldots,Z_k)$ is $\cA(Z_1,\ldots,Z_k)$ with the vector $z$ substituted for the variables $x$.
\end{lemma}
\begin{proof}
  By SoS Cauchy-Schwarz it suffices to show $\pE \|x - z\|^2 \leq \max_{\pE'\text{ satisfies } \cB(z,Z_1,\ldots,Z_k)} \pE\nolimits' \|z - y\|^2$ where $\pE$ is the minimizer of \cref{def:sos-median}.
  Since $\pE$ is the $\arg \min$, this bound follows from comparing $\pE$ to the distribution placing all mass on the vector $z$.
\end{proof}

\begin{lemma}\label[lemma]{lem:sos-med-2}
  Let $Z_1,\ldots,Z_k \in \R^d$ be i.i.d. copies of a random variable $Z$ with mean $\E Z = \mu$ and covariance $\E(Z-\mu)(Z-\mu)^\top = \Sigma$.
  Let $\cB$ be the polynomial system of \cref{lem:sos-med-1}.
  With probability at least $1 - \exp(k/32)$,
  \[
    \max_{\substack{\pE \text{ satisfies}\\ \cB(\mu,Z_1,\ldots,Z_k)}} \pE \|\mu - y\|^2 \leq 1024 \Paren{ \frac{\Tr \Sigma}{k} + \|\Sigma\|}\mper
  \]
\end{lemma}
We prove \cref{lem:sos-med-2} in the next section.
Now we are prepared to prove the main theorem.

\begin{proof}
  Each of the vectors $Z_i$ computed in \textsc{EstimateMean} is the average of $\tfrac n {32 \log(1/\delta)}$ vectors $X_j$.
  Thus if $\E X = \mu$ and $\E (X - \mu)(X - \mu)^\top = \Sigma$, then $\E Z_i = \mu$ and $\E (Z_i - \mu)(Z_i - \mu)^\top = \tfrac{32 \log(1/\delta)}{n} \Sigma$.
  Also, $Z_1,\ldots,Z_k$ are independent.
  By \cref{lem:sos-med-2}, with probability $1-\delta$ over $Z_1,\ldots,Z_k$ 
  \[
  \max_{\substack{\pE \text{ satisfies}\\ \cB(\mu,Z_1,\ldots,Z_k)}} \pE \|\mu - y\|^2 \leq 1024 \Paren{ \frac{\Tr \Sigma}{n} + \frac{32 \|\Sigma\| \log(1/\delta)}{n} }\mper
  \]
  The main theorem now follows from \cref{lem:sos-med-1}.
\end{proof}



\fi

